Runtime-Safety-Guided Policy Repair

We study the problem of policy repair for learning-based control policies in safety-critical settings. We consider an architecture where a high-performance learning-based control policy (e.g. one trained as a neural network) is paired with a model-based safety controller. The safety controller is endowed with the abilities to predict whether the trained policy will lead the system to an unsafe state, and take over control when necessary. While this architecture can provide added safety assurances, intermittent and frequent switching between the trained policy and the safety controller can result in undesirable behaviors and reduced performance. We propose to reduce or even eliminate control switching by `repairing' the trained policy based on runtime data produced by the safety controller in a way that deviates minimally from the original policy. The key idea behind our approach is the formulation of a trajectory optimization problem that allows the joint reasoning of policy update and safety constraints. Experimental results demonstrate that our approach is effective even when the system model in the safety controller is unknown and only approximated.

==> ana.tex <==
\section{Theoretical Analysis for Nonlinear Case}

As the algorithm adopts local linearization and supervised learning on the manifold of the policy parameters, this section will discuss the theoretical bounds involved in the highly nonlinear case and clarify certain underlying assumptions that validate those bounds. Firstly, we show that by applying trust region method in the trajectory optimization, the policy update implied by the trajectory update is in a descent direction.

\begin{assumption}
The policy as a function of state and parameters $\pi:X\times \Theta \rightarrow U$ is $\lambda_x$-smooth in $x$ and $\lambda_\theta$-smooth in $\theta$
\end{assumption}

%\begin{assumption}
%The neural policy $\pi:X\times \Theta \rightarrow U$ is $\lambda_x$-weakly convex in $x$ and $\lambda_\theta$-smooth in $\theta$. 
%\end{assumption}

The assumption implies that for any $x,\delta x\in X$ and $\theta, \delta\theta\in \Theta$, the following inequalities hold.
\begin{eqnarray}
\pi_{\theta +\delta\theta}(x + \delta x) - \pi_\theta(x)&\leq& \delta x^T \nabla_x\pi_\theta(x) + \delta\theta^T \nabla_\theta\pi_\theta(x) + \frac{\lambda_x}{2}||\delta x||^2_2 + \frac{\lambda_\theta}{2} ||\delta\theta||^2_2\nonumber\\\label{smooth}\\

\pi_{\theta +\delta\theta}(x + \delta x) - \pi_\theta(x)&\geq& \delta x^T \nabla_x\pi_\theta(x) + \delta\theta^T \nabla_\theta\pi_\theta(x) - \frac{\lambda_x}{2}||\delta x||^2_2 - \frac{\lambda_\theta}{2} ||\delta\theta||^2_2\nonumber\\\label{wconv}
\end{eqnarray}

\begin{assumption}
The policy as a function of state and parameters $\pi:X\times \Theta \rightarrow U$ is $L_x-$Lipschitz continuous over $x$ and $L_\theta-$Lipschitz continuous over $\theta$.
\end{assumption}

The assumption implies that for any $x,\delta x\in X$ and $\theta, \delta\theta\in \Theta$, the following inequalities hold.
\begin{eqnarray}
||\pi_{\theta +\delta\theta}(x + \delta x) - \pi_\theta(x)||&\leq& L_x||\delta x|| + L_\theta||\delta\theta||\label{lip}
\end{eqnarray}

When a policy parameter update $\theta \rightarrow \theta + \delta\theta$ happens. It induces a set of trajectory updates from $\{\tau\}\sim \pi_\theta$ to $\{\tau + \Delta\tau\}\sim\pi_{\theta + \Delta \theta}$. We prove that by using trust region approach to bound the trajectory state update $|\delta x|\leq \Delta_x$ and policy parameter update $|\delta\theta|\leq \Delta_\theta$, the policy update is guaranteed to reduce the loss under certain conditions.

\begin{proposition}
Given data set $\Gamma=\{(x, u)\}\sim \pi_\theta$, $\forall \delta\theta, s.t. ||\delta\theta||\leq \Delta_\theta$, $J_\Gamma(\pi_{\theta + \delta\theta})-J_\Gamma(\pi_\theta)\leq 0$ if $\forall (x, u)\in\Gamma, \delta x^T Q_x + \delta u^T Q_u\leq -\frac{L^2_\theta\Delta_\theta^2}{2}-\frac{||\nabla_\pi l_{x,\pi_\theta}||}{2} (\lambda_x\Delta_x + \lambda_\theta\Delta_\theta)$ where $||\delta x||\leq \Delta_x$ and $Q_x, Q_u$ are defined in (\ref{_LP})(\ref{LP_}).
\end{proposition}

\begin{proof}
Note that $l_{x,\pi_{\theta}}=\frac{1}{2}||\pi_{\theta_0}(x)-\pi_{\theta}(x)||^2_2$ is convex in $\pi_{\theta}(x)$ and $\nabla^2_{\pi\pi}
l_{x,\pi_\theta}\equiv I$.

\resizebox{.91\linewidth}{!}{
  \begin{minipage}{\linewidth}
\begin{eqnarray}
&&J_{\Gamma}(\pi_{\theta + \delta\theta})-J_{\Gamma}(\pi_\theta)\nonumber\\
&\equiv& \mathbb{E}_{(x, u)\sim \Gamma}[(\pi_{\theta+\delta\theta}(x) -\pi_\theta(x))^T\nabla_\pi
l_{x,\pi_\theta}+\frac{1}{2}(\pi_{\theta+\delta\theta}(x) -\pi_\theta(x))^T \nabla^2_{\pi\pi}
l_{x,\pi_\theta} (\pi_{\theta+\delta\theta}(x) -\pi_\theta(x))]\nonumber\\
&=&\mathbb{E}_{(x, u)\sim \Gamma}[\frac{1}{2}(\pi_{\theta+\delta\theta}(x) -\pi_\theta(x))^T(\pi_{\theta+\delta\theta}(x)-\pi_{\theta}(x)) + (\pi_{\theta+\delta\theta}(x) -\pi_\theta(x))^T\nabla_\pi l_{x,\pi_\theta}]\nonumber\\
&\leq&\mathbb{E}_{(x, \cdot)\sim \Gamma}[\frac{L^2_\theta\Delta_\theta^2}{2}+(\delta u- \delta x^T\nabla_x \pi_{\theta}(x))^T\nabla_\pi l_{x,\pi_\theta} + \nonumber\\
&&\frac{1}{2}max((\lambda_x||\delta x||^2_2+ \lambda_\theta||\delta\theta||^2_2)\nabla_\pi l_{x,\pi_\theta}, (-\lambda_x||\delta x||^2_2 - \lambda_\theta||\delta\theta||^2_2)\nabla_\pi l_{x,\pi_\theta}
]\nonumber\\  
&=& \mathbb{E}_{(x, \cdot)\sim \Gamma}[\frac{L^2_\theta\Delta_\theta^2}{2}+ \delta u^T Q_u + \delta x^T Q_x+\frac{||\nabla_\pi l_{x,\pi_\theta}||}{2}(\lambda_x\Delta_x + \lambda_\theta\Delta_\theta) ]\label{descent}
\end{eqnarray}
\end{minipage}
}

Since (\ref{descent}) is negative, $\delta\theta$ is a descent direction. The proof is complete.
\end{proof}

This bound implies that during the trajectory optimization, in addition to enforcing a trust region constraint on $\delta x$, line search should be applied to ensure that the loss is sufficiently decreased in the trajectory manifold to guarantee a descent direction on the policy manifold. Note that since (\ref{descent}) also involves $\Delta_\theta$, trust region constraint should be considered not only in the trajectory optimization step but also in the policy fitting step.

==> app.tex <==
\newpage
\section*{Appendix}

\textbf{Theorem 1.} Given a $\langle\pi_{\theta_0},\pi_{safe}\rangle$ pair, let $\epsilon_{1}, \epsilon_2$ and $\epsilon_3$ be the probability of $\langle\pi_{\theta_0},\pi_{safe}\rangle$ generating a $H$-length trajectory where $\pi^{safe}(x, \pi_{\theta_0}(x))\neq \pi_{\theta_0}(x)$ happens in at least one, two and three states respectively. 
Then, $\eta(\pi^{safe}) - \eta(\pi_{\theta_0})  \leq \epsilon_1 H  + \epsilon_2 (H-1)+ \frac{\epsilon_3(H-1)H}{2}$.

\begin{proof}
Define $e(x)\in\{0, 1\}$ as the probability of the safety controller intervening in state $x$. Let $p_{<t}$ represent the probability of the safety controller never intervening before step $t$. Then we use $d_t(x_t, u_t)$ to represent the probability of generating $x_t, u_t$ at step $t$ conditioned on $p_{<t}$, while using $d'_t(x_t, u_t)$ to represent the probability  of generating $x_t, u_t$ at step $t$ but conditioned on $1-p_{<t}$. Let $p_{>t}$ be the probability of the safety controller never intervening after step $t$ conditioned on the fact that the safety controller intervenes not only at step $t$ and also for at least one time before step $t$. Then obviously $\epsilon_1 = \sum^H_{t=0} p_{<t}\mathbb{E}_{(x_t, u_t)\sim d_t} [e(x_t)]$, $\epsilon_2 = \sum^{H}_{t=1} (1 - p_{<t})\mathbb{E}_{(x_t, u_t)\sim d'_t} [e(x_t)]p_{>t}$ and $\epsilon_3\geq (1 - p_{<t})\mathbb{E}_{(x_t, u_t)\sim d'_t} [e(x_t)](1-p_{>t})\ \forall t\in\{0, 1, 2, \ldots, H\}$. Note that $A_{\pi_{\theta_0}}(x_t, u_t) = 0$ in states where $u_t = \pi^{safe}(x_t, \pi_{\theta_0}(x_t))=\pi_{\theta_0}(x_t)$ while  $A_{\pi_{\theta_0}}(x_t, u_t) \geq 0$ in states where $u_t = \pi^{safe}(x_t, \pi_{\theta_0}(x_t))\neq\pi_{\theta_0}(x_t)$ due to the optimality of $\pi_{\theta_0}$ under the current cost function $c$. In addition, $A_{\pi_{\theta_0}}(x_t, u_t)\leq (H-t)(\underset{x\in X}{\max}\ c(x) - \underset{x\in X}{\min}\ c(x))=H-t$ for all $x_t\in X, t\in\{0, 1, \ldots, H\}$. Then we use those facts and assumptions to derive the theorem as below based on (\ref{trpo}).\end{proof}

\resizebox{.91\linewidth}{!}{
\begin{minipage}{\linewidth}
\begin{eqnarray}
&&\eta(\pi^{safe})\nonumber\\
&=&\eta(\pi_{\theta_0}) + \mathbb{E}_{\tau\sim\pi^{safe}}[\sum^H_{t=0}A_{\pi_{\theta_0}}(x_t, u_t)]\nonumber\\
&=& \eta(\pi_{\theta_0}) + \sum^H_{t=0}\mathbb{E}_{x_t, u_t\sim\pi^{safe}}[e(x_t)A_{\pi_{\theta_0}}(x_t, u_t)]\nonumber\\
&=& \eta(\pi_{\theta_0}) + \sum^H_{t=0}p_{<t}\mathbb{E}_{x_t, u_t\sim d_t} [ e(x_t)A_{\pi_{\theta_0}}(x_t, u_t)]  + \sum^H_{t=1} (1 - p_{<t})\mathbb{E}_{x_t, u_t\sim d'_t}[e(x_t) A_{\pi_{\theta_0}}(x_t, u_t)]p_{>t} \nonumber\\
&& +  \sum^{H-1}_{t=1}(1 - p_{<t})\mathbb{E}_{x_t, u_t\sim d'_t}[e(x_t)A_{\pi_{\theta_0}}(x_t, u_t)](1 - p_{>t}) \nonumber\\
&\leq& \eta(\pi_{\theta_0}) + \sum^H_{t=0}p_{<t}\mathbb{E}_{x_t, u_t\sim d_t} [ e(x_t)(H-t)]  + \sum^H_{t=1} (1 - p_{<t})\mathbb{E}_{x_t, u_t\sim d'_t}[e(x_t) (H-t)p_{>t}]\nonumber\\
&&+  \sum^{H-1}_{t=1} (H-t)\epsilon_3 \nonumber\\
&\leq& \eta(\pi_{\theta_0}) + H \sum^H_{t=0}p_{<t}\mathbb{E}_{x_t, u_t\sim d_t} [ e(x_t)]  + (H-1)\sum^H_{t=1} (1 - p_{<t})\mathbb{E}_{x_t, u_t\sim d'_t}[e(x_t)p_{>t}]+  \sum^{H-1}_{t=1} (H-t)\epsilon_3 \nonumber\\
&\leq& \eta(\pi_{\theta_0}) + \epsilon_1 H  + \epsilon_2 (H-1)+ \frac{\epsilon_3(H-1)H}{2}
\end{eqnarray}
\end{minipage}
}

